An Efficient Inference Framework for Early-exit Large Language Models

Building efficient inference framework has gained increasing interests for research community. Early-exit models, a variant of LLMs, improves the inference efficiency of LLMs by skipping rest layers and directly generate output tokens when they are confident enough. However, there is no work of LLM inference framework that takes early-exit models into consideration. This is non-trivial as prior art on LLM inference cannot be directly applied to early-exit models. In this work, we solves two key challenges in building efficient inference framework for early-exit models: (1) batch inference at iteration-level granularity; and (2) KV cache management. For the former, we propose to process the batch until all sequences surpass the early-exit confidence threshold. For the latter, we propose to fill the KV cache of rest layers before the iteration terminates. Our evaluation shows that, compared with the original vLLM operating at full layers, our solution achieves up to 1.25x speed up.

==> table/algorithm.tex <==
\begin{algorithm}[t!]
{
\renewcommand\baselinestretch{0.8}\selectfont
\caption{Update operation of \lru{}.}
\KwIn{key array $\texttt{key}[1\cdots n]$, value array $\texttt{val}[1\cdots n]$, cache state $S_{lru}=\begin{pmatrix}1&\cdots& n\\p_1&\cdots &p_n\end{pmatrix}$, key-value pair $\langle k, v\rangle$ for insertion.}
\label{code:lru}

$\langle k_e, i\rangle=\texttt{Update\_Key\_Array}(\texttt{key}, k)$\;
$S_{lru}=\texttt{Update\_Cache\_State}(S_{lru}, i)$\;
\uIf{$k_e = k$} {
    $\texttt{Update\_Value}(\texttt{val}, S_{lru}(1), v)$\;
}
\Else {
    $\texttt{Replace\_Value}(\texttt{val}, S_{lru}(1), v)$\;
}

\SetKwFunction{FMain}{Update\_Key\_Array}
\SetKwProg{Fn}{Function}{:}{end}
\Fn{\FMain{$\texttt{key}[], k$}}{
    $k_e\gets k$\;
    \For{$i=1\to n$} {
        Swap$(k_e, \texttt{key}[i])$\;
        \If{$k_e = k$} {
            \Return $\langle k, i\rangle$\;
        }
    }
    \Return $\langle k_e, n\rangle$\;
}
\SetKwFunction{FMain}{Update\_Cache\_State}
\SetKwProg{Fn}{Function}{:}{end}
\Fn{\FMain{$S_{lru}, i$}}{
    \Return 
    $\begin{pmatrix} 1 & 2 & \cdots & i & i + 1 & \cdots & n \\ i & 1 & \cdots & i - 1 & i + 1 & \cdots & n \end{pmatrix}
    \times S_{lru}$\;
}
\SetKwFunction{FMain}{Update\_Value}
\SetKwProg{Fn}{Function}{:}{end}
\Fn{\FMain{$\texttt{val}[], i, v$}}{
    $\texttt{val}[i]=$Update$(\texttt{val}[i], v)$\;
}
\SetKwFunction{FMain}{Replace\_Value}
\SetKwProg{Fn}{Function}{:}{end}
\Fn{\FMain{$\texttt{val}[], i, v$}}{
    $\texttt{val}[i]=v$\;
}
}
\end{algorithm}

==> table/table.tex <==
\begin{table}[t!]
\centering
%
\caption{Hardware resources used by \plru{} systems.}
%
\begin{tabular}{|l|rrr|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Resource}}} & \multicolumn{3}{c|}{\textbf{Percentage}}                                                             \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{\sysa} & \multicolumn{1}{c|}{\sysb} & \multicolumn{1}{c|}{\sysc} \\ \hline
Hash Bits                                       & \multicolumn{1}{r|}{7.55\%}   & \multicolumn{1}{r|}{10.82\%}  & 3.97\%                      \\
SRAM                                            & \multicolumn{1}{r|}{11.25\%}  & \multicolumn{1}{r|}{14.09\%}  & 24.90\%                     \\
Map RAM                                         & \multicolumn{1}{r|}{18.58\%}  & \multicolumn{1}{r|}{23.21\%}  & 41.23\%                     \\
TCAM                                            & \multicolumn{1}{r|}{0\%}      & \multicolumn{1}{r|}{0\%}      & 0\%                         \\
Stateful ALU                                    & \multicolumn{1}{r|}{14.58\%}  & \multicolumn{1}{r|}{20.83\%}  & 17.71\%                     \\
VLIW instr                                      & \multicolumn{1}{r|}{6.25\%}   & \multicolumn{1}{r|}{6.64\%}   & 4.17\%                      \\ \hline
\end{tabular}
%
% \begin{minipage}{0.33\textwidth}
% \centering
% \begin{tabular}{|m{0.33\columnwidth}|m{0.14\columnwidth}<{\raggedleft}|m{0.26\columnwidth}<{\raggedleft}|}
% \hline
% \textbf{Resource}   & \textbf{Usage} & \textbf{Percentage} \\ \hline
% Hash Bits     & 377      & 7.55\%            \\
% SRAM          & 108      & 11.25\%           \\
% Map RAM       & 107      & 18.58\%           \\
% TCAM          & 0        & 0\%               \\
% Stateful ALU  & 7        & 14.58\%           \\
% VLIW instr    & 24       & 6.25\%            \\
% \hline
% \multicolumn{3}{c}{(a) \sysa{} system (one pipeline).} \\
% \end{tabular}
% \end{minipage}
% %
% \begin{minipage}{0.33\textwidth}
% \centering
% \begin{tabular}{|m{0.33\columnwidth}|m{0.14\columnwidth}<{\raggedleft}|m{0.26\columnwidth}<{\raggedleft}|}
% \hline
% \textbf{Resource}   & \textbf{Usage} & \textbf{Percentage} \\ \hline
% Hash Bits     & 2160     & 10.82\%          \\
% SRAM          & 541      & 14.09\%          \\
% Map RAM       & 536      & 23.21\%          \\
% TCAM          & 0        & 0\%              \\
% Stateful ALU  & 40       & 20.83\%          \\
% VLIW instr    & 102      & 6.64\%           \\
% \hline
% \multicolumn{3}{c}{(b) \sysb{} system (four pipelines).} \\
% \end{tabular}
% \end{minipage}
% %
% \begin{minipage}{0.33\textwidth}
% \centering
% \begin{tabular}{|m{0.33\columnwidth}|m{0.14\columnwidth}<{\raggedleft}|m{0.26\columnwidth}<{\raggedleft}|}
% \hline
% \textbf{Resource}   & \textbf{Usage} & \textbf{Percentage} \\ \hline
% Hash Bits     & 396      & 3.97\%           \\
% SRAM          & 478      & 24.90\%          \\
% Map RAM       & 475      & 41.23\%          \\
% TCAM          & 0        & 0\%              \\
% Stateful ALU  & 17       & 17.71\%          \\
% VLIW instr    & 32       & 4.17\%           \\
% \hline
% \multicolumn{3}{c}{(c) \sysc{} system (two pipelines).} \\
% \end{tabular}
% \end{minipage}
\label{tab:resource}
\end{table}

==> tex/2.3.tex <==
\presub
\subsection{Opportunities and Challenges for Early-exit Model inference}
\label{sec:background:chanllenge}
\postsub

Inspired by Orca, we find there are opportunities in improving the inference efficiency under batch inference. 
Even iteration-level inference technique is not enough for early-exit models, because during the execution of one iteration, some sequences may exit early while other sequences should still go through the rest layers. 
Naive implementation will result in the execution time of one iteration being bottle-necked by the deepest execution layer of the batch, which reduces the benefit of early-exit strategies.
% experimental insights?
Therefore, a more efficient inference system should work at the layer scale, which can reduce the waste of computation utility.

However, it is more challenging to design efficient scheduling algorithms for such fine-grained execution.
%
For the iteration-level scheduling in Orca, the eviction of sequences is to simply evict finished ones, and the replenishment of new sequences can use popular strategies such as FIFO.
%
For the layer-level scheduling, it is challenging to decide which sequences to be run in the next turn is the most efficient.
We choose to run a batch of sequences that are in the same layer, because in such way we can better utilize the parallelism.
Prior work has pointed out that the data transmission between GPU memory and CPU memory is slow and becomes the bottleneck of the inference system \cite{??}.
Therefore, the design goal of our scheduling algorithm is to minimizes the data transmission while improving the computation efficiency.

==> tex/5.3.tex <==
\presub
\subsection{Analysis}
\label{sec:eval:analysis}
\postsub

It is reasonable to see that our solution achieves better performance.
Our solution applies early-exit models, so the decoding process of tokens consumes less number of layers in average, which is consistent with the reduction of inner-token latency.
The application of early-exit models also improves the token generation throughput.

Comparison between three different early-exit mechanisms shows that the one based on the hidden states similarity is the most efficient.
This is reasonable, because different early-exit mechanisms introduce different computation overhead for each layer.
Computing hidden states similarity only involves calculating the cosine function for two batch of vectors, while the classifier and softmax require the hidden states to go through an additional layer.
This may indicate that hidden states similarity-based early-exit techniques are preferable for building efficient inference service.



==> tex/layer-level.tex <==
\presub
\subsection{Layer-level Scheduling}
\postsub
\label{sec:system:schedule}


For layer-level scheduling, each sequence $s$ is associated with a layer index number $l_s$, which records the next layer index that the sequence $s$ should execute at.
We maintain a queue $Q_u$ for those pending sequences that have not executed any inference, and a queue $Q_i$ for those sequences that have run inference at least once.
We also maintain a list $L$ for sequences that are currently stored in the GPU memory.
Note that $L$ is not equivalent to $Q_i$, because some sequences may be evicted from the GPU memory before finished.
In each turn of the inference, we execute inference for sequences with the same layer index number.
%
During the inference of a batch of sequences on a transformer layer, the linear operators such as QKV computation at the beginning and MLP computation at the end can be done at the flatten tensor of the batch, utilizing the parallelism of batch inference.
Only the attention operation should be done at different sequences individually.
%
% Prior work has pointed out that memory exchange between GPU memory and CPU memory is costly.
Then the key question is: how to schedule the execution for a batch of sequences that are stored in the GPU memory?
% When designing the scheduling algorithm, we consider the following two questions. First, how to choose sequences to form a batch in the current schedule? Second, how to design a policy to evict sequences from the GPU memory?


% For the first question, we choose the layer number index associated with most stored sequences in $L$.
% Then the associated stored sequences are selected as the scheduled batch of sequences for running inference.
% %
% For the second question, we use a heuristic strategy for eviction.
% %
% We maintain the average number of layers per turn for the current batch, which serves as the indicator of the computation efficiency.
% %
% If the current batch has run over $\delta$ turns and the metric is lower than $\lambda$, we evict the sequence with the smallest running turns.
% %
% Then we select sequences in $Q_u$ until the GPU memory cannot hold more sequences again. 


We review the process of layer-level scheduling and find that it can be modeled as reinforcement learning.
At each scheduling, the state of the sequence batch stored in the GPU memory is defined as the execution status of the sequences, \eg, the index of execution position and the next execution layer for each sequence.
Based on the state of the batch, we take an action to execute inference on one of the layers.
The goal of the scheduling algorithm is to maximize the utility of computation, and therefore we define the reward as the number of sequences that engage in the current inference, which means their next execution layers match the scheduling layer.
During the execution, each engaged sequence has a probability to exit early, which means its position index increases by 1 and the next execution layer index is set to 1, and otherwise the next execution layer index increases by 1.
The transformation of the state follows the Markov decision process.
A naive solution is to use a greedy strategy: choose the layer number index that matches most sequences in the batch.
However, such strategy may not maximize the computation efficiency in the long term.
With reinforcement learning, we set the discount rate $\lambda \in \left(0, 1\right)$ and denote the reward in $i^{th}$ turn as $R_i$, then the goal is to maximize the long term discounted rewards:
$$R_0 + \lambda R_1 + \lambda^2R_2+ \lambda^3R_3 + ...$$



To reduce the complexity of the state, we only consider the status of the next execution layers for each sequence.
We do not consider those RL algorithms based on neural network because they may lead to huge scheduling overhead. 
We propose two solutions.
% We apply the Q-learning algorithm as it is efficient and accurate, and we propose two solutions:

\bbb{Basic solution:}
In the basic solution, we apply the Q-learning algorithm as it is efficient and accurate.
Q-learning algorithm maintains a Q-table, where $Q(S, a)$ evaluates the expected future return for the action $a$ under the state $S$.
Suppose at the $t^{th}$ turn the state is $S_t$ and we take the action $A_t$, and after the inference the state transforms to $S_{t+1}$, the Q-table is updated according to the following formula:
$$Q(S_{t}, A_t) = Q(S_t, A_t) + \alpha (R_t + \lambda* max_{A'} Q(S_{t+1},A') - Q(S_t, A_t))$$
We initialize the Q-table according to the greedy strategy: the $Q(S, a)$ is set to the number of matched next execution layers.
%在用到时初始化
%overhead
%intuitive explain the q-learning

The shortcoming of the basic solutions is that the maintained states in the Q-table may be unacceptably large.
%
Suppose the number of layers in the model is $L$, and the batch size is $N$, then the number of potential states is $C_{L}^{N+L} = \frac{(N+L)!}{N! * L!}$.
%
For each state, we should maintain at most $L$ values for different layers.
Therefore the memory cost of Q-table is $O(\frac{(N+L)!}{N! * (L-1)!})$
%
For a scenarios where we use the 8-layer CALM model with batch size ???, $\frac{(N+L)!}{N! * (L-1)!} \approx ??$ may be acceptable.
%
But if the batch size is large, \eg, in VLLM \cite{??} the batch size may be around $100$, then maintaining Q-table is impossible, and we need TODO solution.

\bbb{TODO solution:}
When maintaining Q-table in memory becomes unacceptable, we can use linear functions to approximate Q-table.
%
The idea is that each state can be represented as a vector $<v_1, v_2, ..., v_L>$, where $v_i$ indicates the number of sequences to be processed in the $i^{th}$ layer.
%
We can use different linear functions to estimate evaluation value on different layers.
%
We maintain a $L \times L$ matrix $M$. For $Q(S, a)$ in the basic solution, we estimate it with $M[a] \cdot V$.
%













